COVID-19 Forecasts Using Internet Search Information in the United States

As the COVID-19 ravaging through the globe, accurate forecasts of the disease spread is crucial for situational awareness, resource allocation, and public health decision-making. Alternative to the traditional disease surveillance data collected by the United States (US) Centers for Disease Control and Prevention (CDC), big data from Internet such as online search volumes has been previously shown to contain valuable information for tracking infectious disease dynamics. In this study, we evaluate the feasibility of using Internet search volume of relevant queries to track and predict COVID-19 pandemic. We found strong association between COVID-19 death trend and the search volume of symptom-related queries such as "loss of taste". Then, we further develop an influenza-tracking model to predict future 4-week COVID-19 deaths on the US national level, by combining search volume information with COVID-19 time series information. Encouraged by the 20% error reduction on national level comparing to the baseline time series model, we additionally build state-level COVID-19 deaths models, leveraging the cross-state cross-resolution spatial temporal framework that pools information from search volume and COVID-19 reports across states, regions and the nation. These variants of ARGOX are then aggregated in a winner-takes-all ensemble fashion to produce the final state-level 4-week forecasts. Numerical experiments demonstrate that our method steadily outperforms time series baseline models, and achieves the state-of-the-art performance among the publicly available benchmark models. Overall, we show that disease dynamics and relevant public search behaviors co-evolve during the COVID-19 pandemic, and capturing their dependencies while leveraging historical cases/deaths as well as spatial-temporal cross-region information will enable stable and accurate US national and state-level forecasts.

==> LitReview.tex <==
Version 1

Few studies have evaluated the contribution of online search queries to modelling COVID-19 cases or death. Most articles analyze the strong correlation between online search behaviors and COVID-19 cases/death time series trend and potential predictive power of the queries, but not closely examining the importance among the search queries nor considering aggregating with other time series information or spatial temporal structures to establish such predictive power. Among those, majority of the articles uses Google Trends data \cite{GoogleTrends} on the topic of monitoring, tracking, and forecasting COVID-19 for several regions: China \cite{li2020retrospective, husnayain2020applications, ARGONet_Baidu}, Europe \cite{mavragani2020tracking, walker2020use}, India \cite{GT_India}, Iran \cite{walker2020use, ayyoubzadeh2020predicting}, U.S. \cite{walker2020use, hong2020population, GT_analysis_US, GT_Analysis_USStates}, Spain \cite{GTStudy_Spain}, and the multiple countries \cite{GT_Analysis_World, Lampos_Media, prasanth2021forecasting}. There are publications using other available internet search data as well, for example Twitter and Youtube searches \cite{rufai2020world}. Among those publications, majority of them focus on studying COVID-19 related search queries' connection to COVID-19 cases/death in different countries and regions using various approaches, including discovering the existences of time delay between search frequencies peaks and COVID-19 trends, various correlation computation and rank analysis between search terms and COVID-19 cases/death \cite{li2020retrospective, husnayain2020applications, GT_analysis_US, prasanth2021forecasting, GTStudy_Spain, GT_Analysis_USStates, GT_Analysis_World, GT_India}. The search queries they investigate and obtain also vary from general COVID-19 related searches that includes ``coronaviours'' or ``COVID'' \cite{li2020retrospective}, to public include interventions and safety precautions such as ``handwashing'' \cite{husnayain2020applications}, and to symptom related searches \cite{GT_Analysis_USStates, walker2020use}.  They all conduct similar connection studies with slight different approaches. For instance, \cite{husnayain2020applications} analyzes COVID-19 related searches in Taiwan; \cite{li2020retrospective} conducts correlation study of internet searches with COVID-19 cases in China; \cite{mavragani2020tracking, GT_Analysis_World} correlates Google Trends data with COVID-19 cases and deaths for different areas; \cite{hong2020population} studies relationships between telehealth searches and COVID-19; \cite{walker2020use} explores the online activity related to ``loss of smell''. Most of them argue for the latent forecast ability of COVID-19 cases/death and potential early detection of outbreaks in their studying areas using such connection \cite{GT_India, GT_Analysis_World, GT_Analysis_USStates}, whereas others take the connection further by applying simple prediction methods \cite{GT_analysis_US, prasanth2021forecasting}. Namely, \cite{GT_analysis_US} demonstrate its selected search queries (potential) predictive power via quantile regression in U.S. states, while \cite{prasanth2021forecasting} uses selected search queries from the connection study with COVID-19 cases/death as input to a vanilla long-short term memory (LSTM) framework for U.S, U.K and India forecasts. Additionally, \cite{ayyoubzadeh2020predicting} takes it further by combining linear regression with vanilla LSTM model to provide short-term COVID-19 cases forecast in Iran. In particular, contrasting to other ad-hoc connection studies and off-the-shelf vanilla forecasting mechanisms, \cite{Lampos_Media} conducted a thorough study on identifying COVID-19 related terms (including popular search terms and symptom related terms), de-noising search frequencies caused by general concerns and media exaggerations, and presenting several future COVID-19 cases/death prediction approaches, including transfer-learning between countries for early detection and Gaussian process for forecasting, which demonstrate search terms' potential explainability to the pandemic. Some articles solely focuses on newly emerged terms during the pandemic, such as \cite{walker2020use}, which investigates ``loss of smell'' related search terms and their importance in understanding COVID-19 disease dynamic, forecast potentials, potential under-recognized COVID-19 symptoms. 

However, none of the publications above thoroughly examine internet searches' predictive power by aggregating with other important information, including COVID-19 time series information, near-by regions/areas spread and etc, and therefore not fully utilizing internet searches power. Solely stating forecast potential and importance of recognizing increasing trend of pandemic related terms is far from enough of understanding the pandemic's dynamics and assist further planning and interventions, as there exist strong connections between search terms and COVID-19 trends in different resolutions (areas). Efficient utilization of various multi-resolution spatial temporal information is needed for different areas' forecasting as there exist connections not only between the related important search terms and COVID-19 trends, but also close-proximity between neighbouring areas'/regions'/countries' spread and public search behaviors.The only internet-search-based model, to the best of our knowledge, that accounts for spatial structure is ARGONet \cite{ARGONet_Baidu}, which uses a clustering and $L_1$-penalized data augmentation technique for 2-day ahead COVID-19 cases forecast in China. So far, none of the existing Internet-search-based methods provide robust weeks-ahead forecasts for different geographical areas in the United States that account for spatial correlations.
\cmtSY{end this paragraph by saying current literature is not enough}



Version 3

The correlation of search engine data (such as Google Trends \cite{GoogleTrends}, Baidu \cite{ARGONet_Baidu}, Twitter, and Youtube searches \cite{rufai2020world}) and the COVID-19 situation has been well documented for multiple countries \cite{GT_Analysis_World, Lampos_Media, prasanth2021forecasting}, including specific studies in China \cite{li2020retrospective, husnayain2020applications}, Europe \cite{mavragani2020tracking, walker2020use}, India \cite{GT_India}, Iran \cite{walker2020use, ayyoubzadeh2020predicting}, U.S. \cite{walker2020use, hong2020population, GT_analysis_US, GT_Analysis_USStates}, and Spain \cite{GTStudy_Spain}. However, these articles mostly focus on the pure correlation exercise, including correlation computation \cite{prasanth2021forecasting, GTStudy_Spain, GT_Analysis_USStates, GT_Analysis_World}, rank analysis \cite{GT_analysis_US}, and cross correlation for time delay between search peaks and COVID-19 cases/deaths \cite{li2020retrospective, husnayain2020applications, GT_India}. None of them examines the importance among the search queries, considers the spatial-temporal structure of the data, or attempts to make weeks-ahead predictions. 

The relevant search queries in existing literature includes general COVID-19 terms such as ``coronaviours'' or ``COVID'' \cite{li2020retrospective}, public safety precautions such as ``handwashing'' \cite{husnayain2020applications}, symptom-related queries such as ``loss of smell'' \cite{GT_Analysis_USStates, walker2020use}. However, most of them focus on a handful of query terms under a specific class, without a large-scale data-driven query identification process. 

While most of existing articles argue for the potential of online search data for COVID-19 forecasts \cite{rufai2020world, li2020retrospective, husnayain2020applications, mavragani2020tracking, walker2020use, hong2020population, GT_India, GT_Analysis_World, GT_Analysis_USStates}, only a few actually build the prediction models \cite{GT_analysis_US, prasanth2021forecasting, ayyoubzadeh2020predicting, Lampos_Media}. They only utilize the temporal information from Google search queries as inputs for model forecasts, including quantile regression \cite{GT_analysis_US}, vanilla long-short term memory (LSTM) framework \cite{prasanth2021forecasting}, linear regression with vanilla LSTM model \cite{ayyoubzadeh2020predicting}, transfer-learning and Gaussian process \cite{Lampos_Media}. 

However, none of the articles above fully utilized the predictive power of internet search data by accounting for the spatial-temporal structure, including the time series information of COVID-19 or internet searches in near-by regions/areas. Other qualitative analysis, ad-hoc correlation exercise, or off-the-shelf model application are even further away from a real impact. Spacial information, in particular, is essential for disease forecasts as nearby ares' spread could directly impact the cases/death growth trend of the current area of interest. Incorporating spatial temporal information has been proven helpful for COVID-19 forecasts in many literature, including in vector autoregressive model \cite{zhu2020high}, and attention based model \cite{jin2021inter}. Google search queries not only have strong correlation with COVID-19 trend (temporal information), nearby areas' Google search and public interests in COVID-19 related terms can directly impact the area of interest's forecasts as well. 

The only internet-search-based model, to the best of our knowledge, that accounts for spatial structure is ARGONet \cite{ARGONet_Baidu}, which uses a clustering and $L_1$-penalized data augmentation technique for 2-day ahead COVID-19 cases forecast in China. So far, none of the existing Internet-search-based methods provide robust weeks-ahead forecasts for different geographical areas in the United States that account for spatial correlations.




